Gaussian Splashing: Direct Volumetric Rendering Underwater

In underwater images, most useful features are occluded by water. The extent of the occlusion depends on imaging geometry and can vary even across a sequence of burst images. As a result, 3D reconstruction methods robust on in-air scenes, like Neural Radiance Field methods (NeRFs) or 3D Gaussian Splatting (3DGS), fail on underwater scenes. While a recent underwater adaptation of NeRFs achieved state-of-the-art results, it is impractically slow: reconstruction takes hours and its rendering rate, in frames per second (FPS), is less than 1. Here, we present a new method that takes only a few minutes for reconstruction and renders novel underwater scenes at 140 FPS. Named Gaussian Splashing, our method unifies the strengths and speed of 3DGS with an image formation model for capturing scattering, introducing innovations in the rendering and depth estimation procedures and in the 3DGS loss function. Despite the complexities of underwater adaptation, our method produces images at unparalleled speeds with superior details. Moreover, it reveals distant scene details with far greater clarity than other methods, dramatically improving reconstructed and rendered images. We demonstrate results on existing datasets and a new dataset we have collected. Additional visual results are available at: https://bgu-cs-vil.github.io/gaussiansplashingUW.github.io/ .

==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------




\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\RD}{\ensuremath{\RR^D}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}
\newcommand{\ellOneNorm}[1]{\norm{#1}_{\ellOne}}





\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}
\newcommand{\WHITE}[1]{{{\color{white}{#1}}}}  

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  
\newcommand{\PURPLE}[1]{{{\color{purple}{#1}}}}  

\newcommand{\gr}[1]{{{\color{gray}{#1}}}}  

\definecolor{brown}{RGB}{165,42,42}
\newcommand{\BROWN}[1]{{{\color{brown}{#1}}}}



\newcommand{\OREN}[1]{\textbf{\MAGENTA{[OREN: #1]}}}
\newcommand{\NIR}[1]{\textbf{\RED{[NIR: #1]}}}
% Make your own
\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}

\newcommand{\REPLACE}[2]{\RED{REPLACE:} \BLUE{#1} \RED{WITH:} \BLUE{#2}}


\newcommand{\SEtwo}{\ensuremath{\mathrm{SE}(2)}}


% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}
\bmdefine\bepsilon{\epsilon}


\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bsigma{\sigma}
\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


 \newcommand{\DP}{\mathrm{DP}}
 \newcommand{\DIR}{\mathrm{Dir}}
 \newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% Method Commands
\newcommand{\cnot}{\mathbf{c}}
\newcommand{\fnot}{\mathbf{f}}
\newcommand{\pnot}{\mathbf{p}}
\newcommand{\signot}{\mathbf{\sigma}}
\newcommand{\munot}{\boldsymbol{\mu}}
\newcommand{\alphanot}{\boldsymbol{\alpha}}
\newcommand{\Signot}{\mathbf{\Sigma}}

\newcommand{\alphai}{\alphanot_i}
\newcommand{\fim}{\fnot_i}
\newcommand{\alphaj}{\alphanot_j}
\newcommand{\fj}{\fnot_j}
\newcommand{\alphak}{\alphanot_k}
\newcommand{\fk}{\fnot_k}
\newcommand{\ci}{\cnot_i}
\newcommand{\Ti}{T_i}
\newcommand{\Tj}{T_j}
\newcommand{\cj}{\cnot_j}
\newcommand{\ck}{\cnot_k}
\newcommand{\mui}{\munot_i}
\newcommand{\sigi}{\signot_i}
\newcommand{\sigj}{\signot_j}
\newcommand{\sigk}{\signot_k}

\newcommand{\Cpixo}{C_{\text{pix}}}
\newcommand{\Cpix}{C_{\text{out}}}
\newcommand{\Cuw}{C_{\text{UW}}}
\newcommand{\Cpixuw}{C_{\text{UWpix}}}
\newcommand{\directv}{B_{\text{d}}}
\newcommand{\directi}{{B_{\text{d}}}_i}
\newcommand{\bsv}{B_{\text{b}}}
\newcommand{\bsvhat}{\widehat{\bsv}}
\newcommand{\bsi}{{B_{\text{b}}}_i}
\newcommand{\lambsi}{{\lambda_{\bsi}}}
%\newcommand{\lambest}{{\lambda_{\text{back-est}}}}
\newcommand{\lambest}{{\lambda_{2}}}

\newcommand{\lossbest}{\Lcal_{\text{bs}}}
%\newcommand{\lambssim}{{\lambda_{\text{D-SSIM}}}}
\newcommand{\lambssim}{{\lambda_{1}}}

\newcommand{\binf}{{B_{\infty}}}
\newcommand{\binfhat}{{\widehat{\binf}}}
\newcommand{\lambbinf}{{\lambda_{\binf}}}
\newcommand{\loss}{\Lcal}
\newcommand{\lossback}{\Lcal_\text{Back}}
\newcommand{\lossbackall}{ \frac{\partial \lossback}{\partial \text{Back}}}


\newcommand{\Sigi}{\Signot_i}
\newcommand{\cmed}{\cnot_{\text{med}}}
\newcommand{\cmedi}{\cnot_{\text{med}_i}}
\newcommand{\cmedj}{\cnot_{\text{med}_j}}
\newcommand{\sigmed}{\signot_{\text{med}}}
\newcommand{\sigmedi}{\signot_{\text{med}_i}}
\newcommand{\sigmedj}{\signot_{\text{med}_j}}
\newcommand{\sigbs}{\signot_{\text{bs}}}
\newcommand{\sigat}{\signot_{\text{att}}}

\newcommand{\ecmedsigmed}{e^{-\cmed\sigmed}}
\newcommand{\eicmedsigmed}{e^{-i\cmed\sigmed}}
\newcommand{\ekcmedsigmed}{e^{-k\cmed\sigmed}}

\newcommand{\sumi}[2][]{\sum_{{#1}=0}^{{#2}}}

\newcommand{\po}[1][]{\text{po}_{#1}}
\newcommand{\power}[1][]{-\frac{1}{2}(\pnot_{#1}-\munot_{#1})^T\Signot{#1}^{-1}(\pnot_{#1}-\munot_{#1})}
\newcommand{\fimpact}{(1-\ecmedsigmed)+\ci\sigi e^{\left(\power[i]\right)}}
\newcommand{\trans}[1][]{\prod_{j=0}^{#1}\left[e^{-(\sigj e^{\left(\power[j]\right)})+\cmed\sigmed}\right]}
\newcommand{\transpo}[1][]{\prod_{j=0}^{#1}\left[e^{-(\sigj e^{\po[j]})+\cmed\sigmed}\right]}

\newcommand{\esummed}[1][]{e^{\sum_{j=0}^{{#1}} -\sigj e^{\po[j]}}}


\newcommand{\z}{\mathbf{z}}
\newcommand{\betad}{\mathbf{\beta}_{D}}
\newcommand{\jc}{\mathbf{J}_{c}}
\newcommand{\bct}{\boldsymbol{B}_{c}^{'}}
